STDArm: Transferring Visuomotor Policies From Static Data Training to Dynamic Robot Manipulation

Recent advances in mobile robotic platforms like quadruped robots and drones have spurred a demand for deploying visuomotor policies in increasingly dynamic environments. However, the collection of high-quality training data, the impact of platform motion and processing delays, and limited onboard computing resources pose significant barriers to existing solutions. In this work, we present STDArm, a system that directly transfers policies trained under static conditions to dynamic platforms without extensive modifications. The core of STDArm is a real-time action correction framework consisting of: (1) an action manager to boost control frequency and maintain temporal consistency, (2) a stabilizer with a lightweight prediction network to compensate for motion disturbances, and (3) an online latency estimation module for calibrating system parameters. In this way, STDArm achieves centimeter-level precision in mobile manipulation tasks. We conduct comprehensive evaluations of the proposed STDArm on two types of robotic arms, four types of mobile platforms, and three tasks. Experimental results indicate that the STDArm enables real-time compensation for platform motion disturbances while preserving the original policy's manipulation capabilities, achieving centimeter-level operational precision during robot motion.

==> chapters/4.method.tex <==
% \section{\sysname}
\section{STDARM}





\subsection{System Overview}
\label{sec:system_overview}
In this section, we will present a system overview from a system process perspective, detailing the data flow from RGB images input and joint motors input to the actual execution of actions. Sec.~\ref{sec:system_overview:policy} introduces the generation of an initial action sequence from observations using the policy network. Sec.~\ref{sec:system_overview:action_manager} elaborates on the management of initial actions at each time step, including temporal ensemble and interpolation strategies. Sec.~\ref{sec:system_overview:stabilizer} provides a brief explanation of the improvements made in transitioning from the above actions to the final executed actions. It is worth mentioning that all these modules are deployed on edge devices without the assistance of external platforms for computation.

\input{fig/pipeline}


\subsubsection{Policy Network}
\label{sec:system_overview:policy}
The policy network $\pi$ is assigned a dedicated process. It continuously retrieves the most recent $n$ steps of observations, including images $\mathcal{I}$ and joint motors $\mathcal{S}$, as input. Based on these observations, the network predicts the action sequence output $\mathbf{u}$ for the next $k$ time steps. Both the observation steps n and prediction steps k are predefined before training. Denoting the actions sequence output as $\mathbf{u}_{t+1:t+k}=\{u_{t+1},...,u_{t+k}\}$, this process can be formulated as:

\begin{equation}
\mathbf{u}_{t+1:t+k} = \pi(\mathcal{I}_{t-n+1:t}, \mathcal{S}_{t-n+1:t})
\end{equation}


\subsubsection{Action Manager}
\label{sec:system_overview:action_manager}
To enable more real-time action outputs on edge devices, we specifically designed an action manager. This module continuously receiving action sequences from the policy network. It maintains an action list $\mathbf{A}=\{A_t, t \in \mathbb{T}\}$, which sequentially contains both recently executed actions and predicted actions yet to be executed. In addition, it maintains corresponding action weights $\mathbf{W}=\{w_t, t \in \mathbb{T}\}$ for performing temporal ensemble. Upon receiving the action sequence $\mathbf{u}_{t_0+1:t_0+k}$ from the policy network, the Action Manager first determines the temporal offset $t_\text{offset}$ based on the prediction's initial time step $t_0$. Using this offset, it updates and manages the action list. The specific equation is as follows:

\begin{equation}
A_t =
\begin{cases}
w^{\text{old}}_{t} \cdot A_t + w^{\text{new}}_t \cdot u_t, & t_0 + t_\text{offset} \leq t \leq |\mathbf{A}|, \\
A_t, & t < t_0 + t_\text{offset}, \\
u_t, & t > |\mathbf{A}|,
\end{cases}
\end{equation}

\noindent where the weights $w^{\text{new}}_{t}$ of $\mathbf{u}_{t_0+1:t_0+k}$ are computed following an exponential distribution parameterized by the hyper parameter $\alpha$. For the Action Manager, the weight of each time step is initialized to 0. After performing temporal ensemble, the weight of each time step is updated by adding the corresponding weight of the predicted action.

\begin{align}
w^{\text{new}}_{t+i} &= \exp(-\alpha i), i \in [0, k] \\
w^{\text{old}}_t &= w^{\text{old}}_t + w^{\text{new}}_{t}
\end{align}

Additionally, considering the relatively low frequency of the policy network's actions sequence output compared to the high frequency required for actual action execution, we perform linear interpolation for actions at finer time step $\tau$. Specifically, for $\tau$ located between $t$ and $t+1$, the interpolated action can be expressed as:

\begin{equation}
A_{\tau} = (\tau - t) A_{t} + (t+1 - \tau) A_{t+1}
\end{equation}

% 线性插值的频率受限于机械臂可以接受的频率和Stabilizer的预测频率


\subsubsection{Stabilizer}
\label{sec:system_overview:stabilizer}
Through the Action Manager, we can obtain high-frequency actions in real time. However, we also need to address the unstable platform's wobble. Considering computation and communication delays, we designed a prediction compensation based stabilizer. This stabilizer predicts platform's wobble over a short future period and modifies the actions to counteract the wobble effectively. Given that we use a camera for SLAM-based localization, this process not only requires real-time wobble prediction but also online optimization of delays and external parameters. Denoting the predicted wobble as $\delta$, the optimized delay as $\Delta t$, and the external parameters as $\mathcal{E}$, the process at finer time step $\tau$ can be expressed as:

\begin{equation}
A'_{\tau} = A_{\tau} + \delta(\tau, \Delta t, \mathcal{E})
\end{equation}



\subsection{Prediction Compensation Based Stabilizer}
\label{sec:stabilizer}
In this section, we provide a detailed description of our prediction compensation-based stabilizer. As previously mentioned, the implementation principally relies on two modules: one module performs real-time wobble prediction, and the other module conducts online optimization of delays and external parameters.

\input{fig/stabilizer}

\subsubsection{pose prediction}
The pose prediction incorporate two parts: a SLAM module and a prediction network. In terms of data flow, we first perform a real-time, high-frequency SLAM-based localization using sensory data from a stereo camera equipped with an IMU to obtain a high-frequency sequence of poses. Then, for each prediction in prediction network $\mathcal{M}$, we use the current pose as the coordinate origin and calculate the sequence of high-frequency pose changes $\Delta P_{-l_0:-1}=\{\Delta p_{-l_0},...,\Delta p_{-1}\}$ from the past $l_0$ frames, which serves as the input to the prediction network. The prediction network directly outputs the future $l_1$ frames' high-frequency pose change sequence $\Delta P_{1:l_1}=\{\Delta p_{1},...,\Delta p_{l_1}\}$. Finally, based on the optimized external parameters $\mathcal{E}$, the delay $\Delta t$, the elapsed time $\Delta t_\tau$ of the predicted action $A_\tau$, and the SLAM's frames per second (fps) $f$, we determine the required changes to the action value. This process is described as follows:

\begin{equation}
\Delta P_{1:l_1} = \mathcal{M}(\Delta P_{-l_0:-1})
\end{equation}

\begin{equation}
\delta(\tau, \Delta t, \mathcal{E}) = 
\mathcal{E}^{-1} \cdot 
(\Delta p_{\lceil-\Delta t_\tau / f \rceil} + 
\Delta p_{\lfloor\Delta t / f \rfloor} ) \cdot 
\mathcal{E}
\end{equation}

Considering the limitation of computational resources and the requirements for system real-time performance, we implement a lightweight prediction network $\mathcal{M}$. Specifically, we parallelized an LSTM and a GRU, which process the same input. We concatenate their corresponding temporal outputs along the feature dimension and finally pass them through a fully connected layer to produce the prediction results, that is:

\begin{equation}
\mathcal{M}(x) = \text{FC}(\text{concat}(\text{LSTM}(x), \text{GRU}(x)))
\end{equation}

\subsubsection{Latency Estimation}
To accurately adjust the actions to be executed based on the future trajectory provided by the trajectory prediction module, we need to design an online delay estimation module. This allows the stabilizer to adaptively select the number of prediction steps to correct the actions according to system delays. To achieve this, We added an end-effector holding task before the robot performed the primary task. Specifically, we printed an additional red marker for the robotic arm to hold in a fixed position. We then used a third-person camera to track the red marker's movement. We conducted a linear search for system delay starting from zero, identifying the delay that minimized the marker's movement as the system delay. To ensure that variations in the robot’s movement did not affect the correctness of the delay estimation, we used the ratio of the speed and position estimator of the red marker on the pixel plane within a certain time frame—measured by the RealSense T265—as the evaluation criterion.

==> fig/enddist.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width = .9\linewidth]{fig/png/enddist.png}
	\caption{enddist
	}
    % \vspace{-1.5em}
	%Examples of \metric and \core.}
	\label{fig:enddist}
\end{figure}

==> fig/show_action_traj.tex <==
\begin{figure}[t]  
    \centering   
    \begin{minipage}[t]{0.48\linewidth}  
        \centering  
        \subfigure[Actions] {\includegraphics[width=\linewidth]{fig/pdf/traj.pdf}} 
    \end{minipage}  
    \hfill   
    \begin{minipage}[t]{0.48\linewidth}  
        \centering  
        \subfigure[Poses] {\includegraphics[width=\linewidth]{fig/pdf/actions.pdf}}  
    \end{minipage}  
    \caption{Actions and Poses\textcolor{red}{what is this?}}  
    % \vspace{-1.5em}
\end{figure}

==> table/ablationstudy.tex <==
\begin{table}[t]
\center
\caption{Ablation Study in Dynamic .}
\label{table:ablation}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
ACT & Action Merge & Lastpose & Stablizer & Image shift & Pick-Put \\ \hline
\checkmark  &              &           &        &             &          \\ \hline
\checkmark  & \checkmark            &           &        &             &          \\ \hline
\checkmark  & \checkmark            & \checkmark         &        &             &          \\ \hline
\checkmark  & \checkmark            & \checkmark         & \checkmark      &             &          \\ \hline
\checkmark  & \checkmark            & \checkmark         & \checkmark      & \checkmark           &          \\ \hline
\end{tabular}
\end{table}

==> table/posepredict.tex <==
\begin{table}[t]
\center
\caption{Pose Predicrt.}
\label{table:posepredicrt}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Latency & 0.2 & 0.4 & 0.6 & 0.8 & 1 \\ \hline
ATE(mm) & 5 & 6  & 7  &  8  & 9  \\ \hline
\end{tabular}
\end{table}

==> table/taskdescribe.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\center
\caption{Task Describe.}
\label{table:three_tasks}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc|cc}
Tasks    & Pick and Put & Stack Cylinder & Get the Delivery & \multicolumn{2}{l}{Drone gets the Delivery} \\ \hline
4DOF Arm 
&  \begin{minipage}[b]{0.35\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/6task1.png}}\end{minipage} 
&  \begin{minipage}[b]{0.35\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/6task2.png}}\end{minipage}  
&  \begin{minipage}[b]{0.35\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/6task3.png}}\end{minipage}   & \multicolumn{2}{l}{\multirow{2}{*}{ \begin{minipage}[b]{0.45\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/uavpick.png}}\end{minipage} }}       \\ \cline{1-4}
6DOF Arm &              &                &                  & \multicolumn{2}{l}{}                       
\end{tabular}}
\end{table*}
